Simulation Based Inference for Efficient Theory Space Sampling: an Application to Supersymmetric Explanations of the Anomalous Muon (g-2)

For the purpose of minimizing the number of sample model evaluations, we propose and study algorithms that utilize (sequential) versions of likelihood-to-evidence ratio neural estimation.We apply our algorithms to a supersymmetric interpretation of the anomalous muon magnetic dipole moment in the context of a phenomenological minimal supersymmetric extension of the standard model, and recover non-trivial models in an experimentally-constrained theory space. Finally we summarize further potential possible uses of these algorithms in future studies.

==> text/cmssm.tex <==


Following the work of \cite{Hollingsworth}, we will demonstrate the efficacy of our approach by approximating the posterior of the Constrained Minimal Supersymmetric Model (cMSSM) and comparing it with Metropolis-Hastings Markov Chain Monte Carlo \cite{mcmc}.

\subsubsection{Background}


\subsubsection{Setup}
In the cMSSM example, $\theta = (m_0,m_{1/2}, A_0,\tan \beta)$ and we choose our observables to be $X = (\Omega_{\textrm{DM}h^2}, m_h)$ where $\Omega_{\textrm{DM}}$ is the dark matter relic density and $m_h$ is the mass of the Higgs boson. We fix the sign of $\mu$ to be positive.  The prior is chosen to be uniform over the parameter ranges specified in table \ref{table:cmssm_parameters}. 
\footnote{We elect to compare against MCMC rather than existing results in the literature due to the large variation of calculated outputs from different softsusy and microMEGAS versions. Comparing microMEGAS evaluations of the two setups on the same sets of parameters we found calculated results with up to $2\%$ discrepancies, a major difference when calculating the Higgs Mass.  We thank the authors of \cite{Hollingsworth} for providing us their calculations which allowed us to discover this disparity.}

Our ensemble is made up of \textbf{XXX} binary classifiers whose inputs are a concatenation of $X$ and $\the ta$ and whose outputs are the logit of the classification probability. Each network has \textbf{XXX} hidden layers with \textbf{XXX} units each, and is trained to minize the BCE loss. During inference time, the ensemble outputs are averaged together to produce approximate likelihood-to-evidence ratio of a given sample. 

Our MCMC is a Markov Chain Monte Carlo (MCMC) algorithm with a Metropolis-Hastings proposal distribution. We use the implementation in emcee with \textbf{XXX} walkers and \textbf{XXX} warmup steps.

\begin{table}[]
    \begin{tabular}{@{}lll@{}}
    \toprule
    Parameter    & Domain          & Description                  \\ \midrule
    $m_0$        & [0, ] TeV       & Universal scalar mass        \\
    $m_{1/2}$    & [0, ] TeV       & Universal gaugino mass       \\
    $A_0$        & $[-X m_0, X m_0]$ & Universal trilinear coupling \\
    $\tan \beta$ & [1.5, X0]       & Ratio of Higgs VEVs          \\ \bottomrule
    \end{tabular}
    \caption{Parameter ranges for the CMSSM.} 
    \label{tab:cmssm_parameters}
\end{table}

\subsubsection{Results}

We compare our approximate posterior with the posterior obtained from MCMC operating on the same likelihood.

\begin{figure}
    \begin{centering}
    \includegraphics[width=0.9\columnwidth]{figures/cMSSM/mcmc_reference_1200000pts.png}
    \caption{Samples from the posterior of the cMSSM obtained with Metropolis-Hastings Markov Chain Monte Carlo algorithm. The MCMC algorithm was run with $1,200,000$ samples, which was the number of samples required for convergence.}
    \label{fig:mcmc_cmssm_posterior}
    \end{centering}
\end{figure}


\begin{figure}
    \begin{centering}
    \includegraphics[width=0.9\columnwidth]{figures/cMSSM/mcmc_posterior_obvervables_corner.png}
    \caption{Observables calculated from samples of the cMSSM posterior obtained with Metropolis-Hastings Markov Chain Monte Carlo. The dashed lines indicate the likelihood we used during inference. We note the distribution of Higgs mass observables has a sharp cutoff at $m_h = 125 \textrm{GeV}$. This is due to the lack of parameter space that can produce large higgs masses.}
    \label{fig:mcmc_cmssm_likelihood}
    \end{centering}
\end{figure}


\begin{figure}
    \begin{centering}
    \includegraphics[width=0.9\columnwidth]{figures/cMSSM/long_LR.png}
    \caption{Samples from the posterior of the cMSSM obtained using SNLR.} 
    \label{fig:LR_cmssm_likelihood}
    \end{centering}
\end{figure}
